Unveiling Implicit Table Knowledge with Question-Then-Pinpoint Reasoner for Insightful Table Summarization

Implicit knowledge hidden within the explicit table cells, such as data insights, is the key to generating a high-quality table summary. However, unveiling such implicit knowledge is a non-trivial task. Due to the complex nature of structured tables, it is challenging even for large language models (LLMs) to mine the implicit knowledge in an insightful and faithful manner. To address this challenge, we propose a novel table reasoning framework Question-then-Pinpoint. Our work focuses on building a plug-and-play table reasoner that can self-question the insightful knowledge and answer it by faithfully pinpointing evidence on the table to provide explainable guidance for the summarizer. To train a reliable reasoner, we collect table knowledge by guiding a teacher LLM to follow the coarse-to-fine reasoning paths and refine it through two quality enhancement strategies to selectively distill the high-quality knowledge to the reasoner. Extensive experiments on two table summarization datasets, including our newly proposed InsTaSumm, validate the general effectiveness of our framework.

==> 050result.tex <==

% We aim to answer the following research questions by evaluating OURS variants with other baselines:
% \begin{itemize}[leftmargin=*,topsep=2pt,itemsep=2pt,parsep=0pt]
% \item \textbf{RQ1}: Does OURS produce better summary compared to standard end-to-end approach?
% \item \textbf{RQ2}: Does OURS more helpful for table summarization compare to other knowledge-aumgented baseline?
% \item \textbf{RQ3}: Does the quality of knowledge generated by OURS ..  
% \end{itemize}
\input{figure_latex/pair_eval_summary_quality}
\input{tables/ood_table}
\subsection{Main Results}

\paragraph{Comparison with end-to-end approach}
We first compare our approach with different variants of end-to-end summary generation.
Table~\ref{tab:main_table} shows that summary conditioned on insights significantly improves the performance of both fine-tuned and zero-shot summarizer. 
From pairwise comparison results in Figure~\ref{fig:pairwise_summary}, we find that summaries conditioned on knowledge from \textsc{QtP} Reasoner tend to be more natural, comprehensive and informative.
% This suggests that augmenting the summarizer with the \textsc{QtP} Reasoner is beneficial not only in enhancing the model's ability to capture related knowledge for the target summary but also in improving the overall quality of the summary.
These suggest that augmenting the summarizer with \textsc{QtP} Reasoner is beneficial in enhancing the model's ability to capture related knowledge for better-quality summary.
In addition, the consistent improvements on different backbone summarizer demonstrates the general effectiveness of our approach. 



\paragraph{Comparison with other reasoner baselines}
We compare \textsc{QtP} Reasoner with other knoweldge-augmented baselines that generate knowledge with two different type of reasoning \textit{i.e.,} step-by-step reasoning(CoT, Plan-and-Solve) and symbolic reasoning(Logical Type, SQL). 
% Figure~\ref{fig:pairwise_summary} shows that summaries grounded to insights are of better quality in all three dimensions compared to the baseline knowledge models. 
% Interestingly, the baseline knowledge models perform even worse than the end-to-end summarizer that does not use additional knowledge.
From Table~\ref{tab:main_table} and Figure~\ref{fig:pairwise_summary}, we observe that incorporating baseline knowledge models into table summarization yields only marginal improvements, and in some metrics, it even underperform when compared to the end-to-end model.
% Especially in faithfulness and insightfulness level metrics, \textsc{QtP} Reasoner outperforms all baselines with average 00\%, 00\%, respectively.
These results indicate that the baseline knowledge models offer limited knowledge, which is insufficient to guide the summarizer in capturing related cues for insightful summarization.
In contrast to this, \textsc{QtP} Reasoner outperfomrs all baselines in most metrics by providing the coarse-to-fine gudiance for required knowledge for the insightful summary.
% which demonstrate the effectiveness of coarse-to-fine knowledge mining process and clear pinpointing of cell evidence while generating the knowledge.


\paragraph{Generalizability of \textsc{QtP} in out-of-domain scenario}
In Table~\ref{tab:ood_table}, we observe that our approach outperforms all baselines in out-of-domain scenarios, where the test domain is unseen during the training phase. This is attributed to \textsc{QtP} Reasoner's generalization ability, which stems from its flexibility of self-questioning the required knowledge from the unseen tables. 
While LLMs show remarkable generalization ability in diverse tasks, we find that they can still benefit from \textsc{QtP} Reasoner in capturing implicit knowledge that provides robust guidance for unseen domains.

% When comparing the results with other knowledge models, \textsc{QtP} Reasoner also excels in most dimensions.
% Specifically, we observe that although logical table operations (Logical Type, SQL) help improve the factual correctness of the summary, it is still limited to generate in-depth knowledge required for scientific summaries in SciGEN, showing low performance in surface-level and insightfulness-level metrics.
Specifically, we find that while logical table operations(Logical Type, SQL) enhance the factual correctness of the summary, it is fall short in providing the insightful knowldege required for scientific summaries in SciGEN. 
% These results emphasize our model's ability to actively extract knowledge from tables without being restricted to specific type of knowledge, making it a versatile reasoner.
We also observe that although the Plan-and-Solve Reasoner shares a similar concept with \textsc{QtP} Reasoner in terms of coarse-to-fine reasoning and achieves comparable performance on surface-level metrics, it still suffers from low faithfulness. 
% This might be due to the multiple stages of operations required to explore the in-depth information from structured tables, where the model is more frequently distracted by irrelevant cues, hindering reliable extraction of knowledge.
% In contrast, our model remains robust against irrelevant information by precisely pinpointing evidence for each insight, leading to a more faithful summarization.
% We posit that this trade-off arises from the multiple stages required to explore in-depth information, where the model is often distracted by irrelevant cues, hindering the reliable extraction of knowledge.  
In contrast, our model remains robust against this insighfulness-faithfulness trade-off by grounding the knowledge mining process to explicitly pinpointed evidence, making it a versatile reasoner. 

% 여러번의 reasoning step을 거치면서도 faithful과 insightful을 모두 놓치지 않는다 를 강조하자 

\subsection{Analysis}
\input{tables/human_eval_knowledge_quality}

% \paragraph{Human evaluation on knolwedge quality} 
\paragraph{\textsc{QtP} produces better-quality knowledge} 
To examine how well \textsc{QtP} Reasoner learns to generate implicit knowledge on table, 
we conduct human evaluation and focus on three dimensions: does the reasoner generate more \textit{diverse}, \textit{insightful} and \textit{faithful} knowledge about table. 
We randomly sample 100 reasoner inferences on the test set of \textsc{InsTaSumm} and ask 3 different human judges to compare the knowledge generated by \textsc{QtP} and other baselines. 
The results are shown in Table~\ref{tab:human_eval_knowledge}.
We can see that .. \textit{text dump text dump ext dump text dump ext dump text dump ext dump text dump ext dump text dump ext dump text dump ext dump text dump ext dump text dump ext dump text dump ext dump text dump ext dump text dump ext dump text dump ext dump text dump ext dump text dump ext dump text dump ext dump text dump text dump text dump ext dump text dump ext dump text dump ext dump text dump ext dump text dump ext dump text dump ext dump text dump ext dump text dump ext dump text dump ext dump text dump ext dump }

\input{tables/ablation_knowledge}
\paragraph{Question guides deeper analysis of the table, while evidence pinpoints faithful cues}
To analyze the role of question and cell evidence, we perform ablation studies to investigate the effects of each component in knowledge generation.
Specifically, we remove all questions from the generated knowledge and train the model to generate fine-level insights with cell evidence, then ablate cell evidence from the training set to train the reasoner to directly predict insights for each question.
The results are shown in Table ~\ref{tab:ablation}. 
We observe that without questions, the summary quality drops signficantly , especially in surface-level and insightfulness-level metrics. When ablating cell evidence, the performance decrease especially in faithfulness-level metrics.  
From these results, we posit that the fine-level question plays crucial role in providing specific guidance to the model for searching in-depth knowledge from the table, while the role of cell evidence is narrowing down the search space with clear pinpointing to avoid distractions from irrelevant cell values.

% Next, we ablate cell evidence from the trainset and train reasoner to directly predict the insight for each question.

% \paragraph{Ablation Study}
% We perform ablation studies focusing on two dimensions to further investigate the effects of each component of our approaches. The results are shown in Table().
% \textbf{(1) Analyze the role of question and cell evidence}: We first ablate aspects and questions from the training set and train reasoner to generate the insights along with the cell evidence.  
% % Specifically, we remove all questions from the generated knowledge and train the model to generate the fine-level insights along with the cell evidence. 
% Next, we ablate cell evidence from the trainset and train reasoner to directly predict the insight for each question.
% \textbf{(2) Analyze the effect of applying knowledge quality enhancement}:
% We reconstruct two different training set by omitting factuality verification in one and importance scoring in the other that are used to train the reasoner. 

% From the table(), we find the follwoing insights: (1):, (2): 


\paragraph{Knowledge quality enhancement leads to better-quality summary} 
To investigate the effect of knowledge quality enhancement strategies, we construct two different training data by omitting factuality verification in one and importance scoring in the other and train different version of reasoner.
The results are shown in Table~\ref{tab:ablation}.
We find that the overall performance decreases when ablating each strategy. 
Specifically, factuality verification impacts more on the faithfulness while importance scoring impacts on the surface and insightfulness metrics. 
Theses results suggest that a quality enhancement strategy for selecting key knowledge that factually aligns with the table is necessary for training a reliable knowledge model.


% \paragraph{Case Study}

% \textit{[text dump text dump text dump text dump text dump text dump text dump text dump text dump text dump text dump text dump text dump text dump text dump text dump text dump text dump text dump text dump text dump text dump text dump text dump text dump text dump text dump text dump text dump text dump text dump text dump text dump text dump text dump text dump text dump text dump text dump text dump text dump text dump text dump text dump text dump text dump text dump text dump text dump text dump text dump text dump text dump text dump text dump text dump]}







==> macro.tex <==
\newcommand{\todoc}[2]{{\textcolor{#1}{#2}}}
\newcommand{\todoblue}[1]{\todoc{blue}{#1}}
% \newcommand{\yeo}[1]{\todoblue{#1}}
% \newcommand{\bwoo}[1]{\todoblue{#1}}

\newcommand{\todocc}[2]{{\textcolor{#1}{[[#2]]}}}
\newcommand{\todored}[1]{\todocc{red}{[[#1]]}}
\newcommand{\hist}[1]{\todored{hist: #1}}

\newcommand\donutemoji{\raisebox{-2pt}{\includegraphics[width=0.9em]{figure/doughnut.png}}}

\newcommand{\todocccc}[2]{{\textcolor{#1}{[[#2]]}}}
\newcommand{\todogreen}[1]{\todocccc{green}{[[#1]]}}
\newcommand{\haejuu}[1]{\todogreen{haejuu: #1}}
\definecolor{mypink1}{rgb}{0.858, 0.188, 0.478}
\newcommand{\yeo}[1]{\textcolor{purple}{#1}}
\newcommand{\dragon}[1]{\textcolor{brown}{#1}}
\newcommand{\bwoo}[1]{\textcolor{olive}{#1}}
\newcommand{\kyle}[1]{\textcolor{blue}{#1}} 
\newcommand{\cheris}[1]{\textcolor{teal}{#1}}
\newcommand{\chatgpt}[1]{\textcolor{gray}{#1}}
\newcommand{\minus}[1]{\textcolor{red}{#1}}
\newcommand{\plus}[1]{\textcolor{ForestGreen}{#1}}
\newcommand{\person}{{$\mathbb{P}$}}
\newcommand{\thought}{$\mathbb{Z}_{\mathbb{P}}$}
\definecolor{olive}{rgb}{0.39, 0.875, 0.12}


\newcommand{\blue}{\textcolor{blue}}
\newcommand{\se}{{\it SE}}%
\newcommand{\eg}{{\it e.g.}}%
\newcommand{\ie}{{\it i.e.}}%
\newcommand{\etal}{{\it et al.}}%
\newcommand{\etc}{{\it etc}}%
\newcommand{\ours}{\textbf{ReMemBot }}%
\newcommand{\memory}{\mathcal{M}}%
\newcommand{\carecall}{$\text{CareCall}_{mem}$}
\newcommand{\acpm}{$\mathbbm{A}^2$-CPM}

\newcommand{\argmin}{\operatornamewithlimits{argmin}}
\newcommand{\argmax}{\operatornamewithlimits{argmax}}
\definecolor{yellow-green}{rgb}{0.3, 0.5, 0.0}

% \newcommand{\concat}{\DOTSB\concat@\slimits@}

% Caligraphy style
\newcommand{\mcal}[1]{{\cal{#1}}}
\newcommand{\calA}{\mbox{${\cal A}$}}
\newcommand{\calB}{\mbox{${\cal B}$}}
\newcommand{\calC}{\mbox{${\cal C}$}}
\newcommand{\calD}{\mbox{${\cal D}$}}
\newcommand{\calE}{\mbox{${\cal E}$}}
\newcommand{\calF}{\mbox{${\cal F}$}}
\newcommand{\calG}{\mbox{${\cal G}$}}
\newcommand{\calH}{\mbox{${\cal H}$}}
\newcommand{\calI}{\mbox{${\cal I}$}}
\newcommand{\calJ}{\mbox{${\cal J}$}}
\newcommand{\calK}{\mbox{${\cal K}$}}
\newcommand{\calL}{\mbox{${\cal L}$}}
\newcommand{\calM}{\mbox{${\cal M}$}}
\newcommand{\calN}{\mbox{${\cal N}$}}
\newcommand{\calO}{\mbox{${\cal O}$}}
\newcommand{\calP}{\mbox{${\cal P}$}}
\newcommand{\calQ}{\mbox{${\cal Q}$}}
\newcommand{\calR}{\mbox{${\cal R}$}}
\newcommand{\calS}{\mbox{${\cal S}$}}
\newcommand{\calT}{\mbox{${\cal T}$}}
\newcommand{\calU}{\mbox{${\cal U}$}}
\newcommand{\calV}{\mbox{${\cal V}$}}
\newcommand{\calW}{\mbox{${\cal W}$}}
\newcommand{\calX}{\mbox{${\cal X}$}}
\newcommand{\calY}{\mbox{${\cal Y}$}}
\newcommand{\calZ}{\mbox{${\cal Z}$}}

\definecolor{lightblue}{RGB}{224,236,247}
\definecolor{deepblue}{RGB}{9,46,107}
\definecolor{defaultcolor}{gray}{0.9}
\definecolor{green}{RGB}{0, 153, 0}
\newcommand{\olive}{\textcolor{olive}}

% \tcbset{
%   aibox/.style={
%     width=\textwidth,
%     top=10pt,
%     colback=white,
%     colframe=black,
%     colbacktitle=black,
%     enhanced,
%     center,
%     attach boxed title to top left={yshift=-0.1in,xshift=0.15in},
%     boxed title style={boxrule=0pt,colframe=white,},
%   }
%   }
% \newtcolorbox{AIbox}[2][]{aibox,title=#2,#1}
% \tcbset{
%   aiboxsmall/.style={
%     width=0.48\textwidth,
%     top=10pt,
%     colback=white,
%     colframe=black,
%     colbacktitle=black,
%     enhanced,
%     center,
%     attach boxed title to top left={yshift=-0.1in,xshift=0.15in},
%     boxed title style={boxrule=0pt,colframe=white,},
%   }
% }
% \newtcolorbox{AIboxSmall}[2][]{aiboxsmall,title=#2,#1}





\tcbset{
  aibox/.style={
    width=\textwidth,
    top=10pt,
    colback=white,
    colframe=black,
    colbacktitle=black,
    center title,
    fonttitle=\bfseries,
    % attach boxed title to top left={yshift=-0.1in,xshift=0.15in},
    % boxed title style={boxrule=0pt,colframe=white,},
  }
}

\newtcolorbox{AIbox}[2][]{aibox,title=#2,#1}

\tcbset{
  aiboxsmall/.style={
    width=0.48\textwidth,
    top=10pt,
    colback=white,
    colframe=black,
    colbacktitle=black,
    center title,
    fonttitle=\bfseries,
    % attach boxed title to top left={yshift=-0.1in,xshift=0.15in},
    % boxed title style={boxrule=0pt,colframe=white,},
  }
}

\newtcolorbox{AIboxSmall}[2][]{aiboxsmall,title=#2,#1}


